DHYMON: a Continuous Decentralized Hybrid Monitoring Architecture for MANETs

We introduce a novel decentralized monitoring algorithm for mobile ad-hoc networks. This algorithm is a combination of gossip-based and tree-based approaches. Its main feature is on multi root nodes selection which provides an opportunity to obtain more accurate results as it maximizes the coverage of the network. Our proposal relies on a thorough defined algorithm and its efficient and effective implementation. The algorithm is divided in two main parts that are its query procedure and its disseminate procedure. To assess different parameters such as accuracy and convergence time, we conducted experiments with an in-house emulated test bed based on Docker and NS3. To show the effectiveness and scalability of our proposal, we conduct intensive emulations that demonstrate very promising results regarding the gain of accuracy.

==> 04_results/automata.tex <==
\begin{figure}
\centering

\scalebox{0.45}{%
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=5cm,
  thick,main node/.style={circle,fill=blue!20,draw,
  font=\sffamily\small\bfseries,minimum size=8mm}]

  \node[main node] (I) {Initial};
  \node[main node] (Q1) [right of=I,node distance=3.85cm] {Q1};
  \node[main node] (Q2) [below right of=Q1] {Q2};
  \node[main node] (A1) [below of=Q2] {A1};
  \node[main node] (A2) [left of=A1,node distance=4.15cm] {A2};
  \node[main node] (A3) [left of=A2] {A3};

  \path[every node/.style={font=\sffamily\small,
      fill=white,inner sep=1pt}]

    % Right-hand-side arrows rendered from top to bottom to
    % achieve proper rendering of labels over arrows.
  (I) edge [] node[align=center] {$startMonitoring()$/\\$SND Query$\\\\$RCV Query$/\\$SND Query$} (Q1)

  (Q1) edge [] node[align=center] {$RCV QueryACK$/\\$acc(ACK\_IP)$} (Q2)
  %(Q1) edge [bend right=25] node[align=center] [near end] {$timeout()$/\\$SND Aggregate$\\\\$edgeNode()$/\\$SND Aggregate$} (A1)
  (Q1) edge [bend right=25] node[align=center] [near end] {$timeout()$/\\$SND Aggregate$} (A1)

  (Q2) edge [loop left] node[align=center] {$RCV QueryACK$/\\$acc(ACK\_IP)$} (Q2)
  (Q2) edge [] node[align=center] [near end] {$RCV Aggregate$/\\$SND Aggregate$} (A1)

  (A1) edge [] node[align=center] {$timeout()$/\\$SND AggregateRoute$} (A2)

  (A2) edge [] node[align=center] {$timeout()$/\\$SND AggregateForward$} (A3)

  (A3) edge [loop left] node[align=center] {$timeout()$/\\$Aggregate Forward$} (A3)

  
  (A3) edge [bend left=30] node[align=center] {$RCV AggregateACK$/\\$done()$\\\\$emptyForwards()$/\\$error()$} (I)
  (A2) edge [bend left=25] node[align=center] {$RCV AggregateACK$/\\$done()$} (I)
  (A1) edge [bend left=20] node[align=center] [near end] {$RCV AggregateACK$/\\$done()$} (I);

\end{tikzpicture}
}

\caption{State machine definition of our protocol} \label{fig:automata}
\end{figure}







% % Author: Marek Fiser <tikz at marekfiser.cz>
% % MESIF protocol: http://en.wikipedia.org/wiki/MESIF_protocol
% \documentclass[tikz, border=10pt]{standalone}
% \usetikzlibrary{arrows}
% \begin{document}
% \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
%   thick,main node/.style={circle,fill=blue!20,draw,
%   font=\sffamily\Large\bfseries,minimum size=15mm}]

%   \node[main node] (M) {M};
%   \node[main node] (E) [below of=M] {E};
%   \node[main node] (S) [below of=E] {S};
%   \node[main node] (F) [below of=S] {F};
%   \node[main node] (I) [below of=F] {I};

%   \path[every node/.style={font=\sffamily\small,
%       fill=white,inner sep=1pt}]
%     % Right-hand-side arrows rendered from top to bottom to
%     % achieve proper rendering of labels over arrows.
%     (M) edge [loop above] node {PrRd/-, PrWr/-} (M)
%         edge [bend left=60] node[right=1mm] {BusRdX/Flush} (I)
%         edge [bend left=40] node[right=1mm] {BusRd/Flush} (S)
%     (E) edge [loop above] node {PrRd/-} (E)
%         edge [bend left=50] node[right=1mm] {BusRdX/Flush} (I)
%         edge [bend left=30] node[right=1mm] {BusRd/Flush} (S)
%     (S) edge [loop above] node {PrRd/-} (S)
%         edge [loop right] node[right=1mm]  {BusRd/-} (S)
%         edge [bend left=40] node[right=1mm] {BusRdX/Flush} (I)
%     (F) edge [bend left=30] node[right=1mm] {BusRdX/Flush} (I)
        
%     % Left-hand-side arrows rendered from bottom to top to
%     % achieve proper rendering of labels over arrows.
%     (I) edge [bend left=65] node[left=1mm] {PrWr/BusRdX} (M)
%         edge [bend left=55] node[left=1mm] {PrRd/BusRd Ex} (E)
%         edge [bend left=30] node[left=1mm] {PrRd/BusRd} (F)
%     (F) edge [loop above] node {PrRd/-} (F)
%         edge [bend left=50] node[left=1mm] {PrWr/BusRdX} (M)
%         edge [bend left=30] node[left=1mm] {BusRd/Flush} (S)
%     (S) edge [bend left=40] node[left=1mm] {PrWr/BusRdX} (M)
%     (E) edge [bend left=30] node[left=1mm] {PrWr/-} (M);
% \end{tikzpicture}
% \end{document}

==> 04_results/packetDefinition.tex <==
\begin{center}
{\tiny
\begin{lstlisting}[style=json]
{ "type": "query|aggregate|aggregate_route|aggregate_forward",
  "parent": "<parent IP>", "source": "<source IP>",
  "destination": "<destination IP>", "gateway": "<next hop IP>", 
  "timeout": <time in ms>, "timestamp": "<sourceIP + UnixTime>"
  "query": { "function": "<monitoring function>",
    "relaySet": [ "<IPs of the source rely set>" ] },
  "aggregate": { "outcome": "<monitoring result>",    
    "observations": <number of observations> } }
\end{lstlisting}
\vspace{-1em}
}
\end{center}

==> 04_results/parametersTable.tex <==
\begin{table}
  \caption{Scenario 1 parameters}\label{table:scenario1param}
  \vspace{-1em}
  \begin{center}
      \begin{tabular}{| l | l |}
      \hline
      \textbf{Parameter Name} & \textbf{Value} \\ \hline
      Number of nodes & 20, 25, 40, 50  \\ \hline
      Network Space & 400x400, 600x600  \\ \hline
      Network Positioning & Random  \\ \hline
      % Running time & 60s (init time 40s) \\ \hline
      Emulation times & 100 (60s each with init time 40s)  \\ \hline
      Mobility & Random Waypoint Model at 5m/s \\ \hline
      % Mobility Speed & 5m/s  \\ \hline
      \end{tabular}
  \end{center}
  \vspace{-2em}
\end{table}

% \begin{table}
%   \caption{Scenario 2 parameters}\label{table:scenario2param}
%   \vspace{-1em}
%   \begin{center}
%       \begin{tabular}{| l | l |}
%       \hline
%       \textbf{Parameter Name} & \textbf{Value} \\ \hline
%       Number of nodes & 25  \\ \hline
%       Network Space & 500x500  \\ \hline
%       Network Positioning & Random  \\ \hline
%       Running time & 80s (init time 60s) \\ \hline
%       Emulation times & 40  \\ \hline
%       Mobility & Random Waypoint Model  \\ \hline
%       Mobility Speed & 2m/s and 5m/s  \\ \hline
%       \end{tabular}
%   \end{center}
%   \vspace{-2em}
% \end{table}
